Multivariate Business Process Representation Learning utilizing Gramian Angular Fields and Convolutional Neural Networks

Learning meaningful representations of data is an important aspect of machine learning and has recently been successfully applied to many domains like language understanding or computer vision. Instead of training a model for one specific task, representation learning is about training a model to capture all useful information in the underlying data and make it accessible for a predictor. For predictive process analytics, it is essential to have all explanatory characteristics of a process instance available when making predictions about the future, as well as for clustering and anomaly detection. Due to the large variety of perspectives and types within business process data, generating a good representation is a challenging task. In this paper, we propose a novel approach for representation learning of business process instances which can process and combine most perspectives in an event log. In conjunction with a self-supervised pre-training method, we show the capabilities of the approach through a visualization of the representation space and case retrieval. Furthermore, the pre-trained model is fine-tuned to multiple process prediction tasks and demonstrates its effectiveness in comparison with existing approaches.

==> sections/backup.tex <==
\begin{mydefinition}{Event log, case, event and attribute} \label{defintion:event_log}
	\\%Let $\mathcal{E}$ be the set of all events, $\mathcal{C}$ be the set of all cases and $\mathcal{L}$ be the event log.
	An event $e \in \mathcal{E}$ is a set of attributes identifying an action in a business process.
	A sequence of events $c = \langle e_1, e_2, ..., e_n \rangle$ is called case $c \in \mathcal{C}$ where $e_{t}$ denotes the t-th event in $c$.
	An event log is a ordered set $\mathcal{L} \subseteq \mathcal{C}$ of cases. 
	%where $c_{n}$ is the n-th case in $\mathcal{L}$.
	%$c_{1}$ is the case with ID 1 and $c_{m}$ case with ID m.
	Each event $e$ refers to exactly one case $c$.\\
	Let $\mathcal{A^{*}}$ be the universe of attributes and $\mathcal{A}$ be the set of all attributes in $\mathcal{L}$. 
	Let $\mathcal{V}$ be the set of values in $\mathcal{L}$.
	Let $E$ be the event attributes and $\mathscr{C}$ be the case attributes where $E \cup \mathscr{C} = \mathcal{A}$.
	Each $a \in E$ is a function $a: \mathcal{E} \mapsto \mathcal{V}$ and each $a \in \mathscr{C}$ is a function $a: \mathcal{C} \mapsto \mathcal{V}$.
	Each function $a$ assigns the value $v \in \mathcal{V}$ either to the t-th event $a(e_{t}) = v$ or to one case $a(c) = v$.\\
	%v_{a}^{e_{t}}$
	%The function $a(e_{t}) = v_{a}^{e_{t}}$ assigns a attribute value to an event while $a(c) = v_{c}$ assigns a attribute value to a case with $v \in \mathcal{V}$.
	Using this, $c_{a} = \langle a(e_1), a(e_2), ..., a(e_n) \rangle$ defines the sequence of attribute values $a$ from case $c$. 
	%Therefore $\mathcal{C}_{a} = \{c_{a}|c \in \mathcal{C}\}$ is the set of all those sequences.
	$\mathcal{V}_{a}$ denotes the set of all attributes values for attribute $a$ in $\mathcal{L}$.
	%and $\mathcal{L}_{a_{i}} = \{\mathcal{C}_{a_{i}}\}$ the event log which only consists of those cases.
	The number of cases in a event log is $|\mathcal{L}|$ and the number of attributes is $|\mathcal{A}|$.
\end{mydefinition}
Examples for frequently and commonly used attributes are:
\begin{itemize}
    \item \textit{case-id(c)} is the case ID of case $c \in \mathcal{C}$.
	\item \textit{activity(e)} is the activity name of event $e \in \mathcal{E}$.
	\item \textit{resource(e)} is the resource of event $e \in \mathcal{E}$.
	\item \textit{time(e)} is the timestamp associated to an event $e \in \mathcal{E}$.
\end{itemize}



Version 2:
\begin{mydefinition}{Event} \label{defintion:event_log}\\
    %Let $\mathcal{E}$ be the set of all events and 
    Let $\mathcal{A^{*}}$ be the universe of attributes. A event $e \in \mathcal{E}$ is characterized as a tuple of event attributes $a \in E \subseteq \mathcal{A^{*}}$.
\end{mydefinition}

%Each function $a \in \mathcal{A}$ assigns a value to the t-th event $a(e_t)$ or to a case $a(c)$.

\begin{mydefinition}{Case and Event Log}\\
    %Let $\mathcal{C}$ be the set of all cases and $\mathcal{L}$ be the event log. 
    %Let $\mathcal{A}$ be the set of all attributes $\mathcal{A^{*}}$ in $\mathcal{L}$, $E \in \mathcal{A}$ be the event attributes and $\mathscr{C} \in \mathcal{A}$ be the case attributes where $E \cup \mathscr{C} = \mathcal{A}$.\\
    A sequence of events $c = \langle e_1, e_2, ..., e_n \rangle$ is called case where $e_{t} \in \mathcal{E}$ denotes the t-th event in $c$. Let $\mathcal{C}$ be the set of all cases.
    An event log $\mathcal{L}$ is a set $\mathcal{L} \subseteq \mathcal{C}$ of cases.
\end{mydefinition}

\begin{mydefinition}{Attributes}\\
    Each event attribute $a \in E$ is a function assigning a value to an event $e \in \mathcal{E}$.
    Cases can also be characterized by case attributes $a \in \mathscr{C} \subseteq \mathcal{A^{*}}$. Each case attribute $a \in \mathcal{A^{*}}$ is a function assigning a value to a case $c \in \mathcal{C}$.\\
	Using this, $c_{a} = \langle a(e_1), a(e_2), ..., a(e_n) \rangle$ defines the sequence of attribute values for a case $c \in \mathcal{C}$ and attribute $a \in E$.
\end{mydefinition}
%\begin{mydefinition}{Attributes} \label{defintion:event_log}\\
    %Let $\mathcal{V}$ be the universe of values.
	%Each $a \in E$ is a function $a: \mathcal{E} \mapsto \mathcal{V}$ and each $a \in \mathscr{C}$ a function $a: \mathcal{C} \mapsto \mathcal{V}$.
%\end{mydefinition}
Examples for frequently and commonly used attributes are:
\begin{itemize}
    \item \textit{case-id(c)} is the case ID of case $c \in \mathcal{C}$.
	\item \textit{activity(e)} is the activity name of event $e \in \mathcal{E}$.
	\item \textit{resource(e)} is the resource of event $e \in \mathcal{E}$.
	\item \textit{time(e)} is the timestamp associated to an event $e \in \mathcal{E}$.
\end{itemize}

==> sections/foundation_definition_old.tex <==


\begin{mydefinition}{Event} \label{defintion:event_log}\\
    %Let $\mathcal{E}$ be the set of all events and 
    Let $\mathcal{A^{*}}$ be the universe of attributes. A event $e \in \mathcal{E}$ is characterized as a tuple of event attributes $a \in E \subseteq \mathcal{A^{*}}$.
\end{mydefinition}

%Each function $a \in \mathcal{A}$ assigns a value to the t-th event $a(e_t)$ or to a case $a(c)$.

\begin{mydefinition}{Case and Event Log}\\
    %Let $\mathcal{C}$ be the set of all cases and $\mathcal{L}$ be the event log. 
    %Let $\mathcal{A}$ be the set of all attributes $\mathcal{A^{*}}$ in $\mathcal{L}$, $E \in \mathcal{A}$ be the event attributes and $\mathscr{C} \in \mathcal{A}$ be the case attributes where $E \cup \mathscr{C} = \mathcal{A}$.\\
    A sequence of events $c = \langle e_1, e_2, ..., e_n \rangle$ is called case where $e_{t} \in \mathcal{E}$ denotes the t-th event in $c$. Let $\mathcal{C}$ be the set of all cases.
    An event log $\mathcal{L}$ is a set $\mathcal{L} \subseteq \mathcal{C}$ of cases.
\end{mydefinition}

\begin{mydefinition}{Attributes}\\
    Each event attribute $a \in E$ is a function assigning a value to an event $e \in \mathcal{E}$.
    Cases can also be characterized by case attributes $a \in \mathscr{C} \subseteq \mathcal{A^{*}}$. Each case attribute $a \in \mathcal{A^{*}}$ is a function assigning a value to a case $c \in \mathcal{C}$.\\
	Using this, $c_{a} = \langle a(e_1), a(e_2), ..., a(e_n) \rangle$ defines the sequence of attribute values for a case $c \in \mathcal{C}$ and attribute $a \in E$.
\end{mydefinition}
%\begin{mydefinition}{Attributes} \label{defintion:event_log}\\
    %Let $\mathcal{V}$ be the universe of values.
	%Each $a \in E$ is a function $a: \mathcal{E} \mapsto \mathcal{V}$ and each $a \in \mathscr{C}$ a function $a: \mathcal{C} \mapsto \mathcal{V}$.
%\end{mydefinition}
Examples for frequently and commonly used attributes are:
\begin{itemize}
    \item \textit{case-id(c)} is the case ID of case $c \in \mathcal{C}$.
	\item \textit{activity(e)} is the activity name of event $e \in \mathcal{E}$.
	\item \textit{resource(e)} is the resource of event $e \in \mathcal{E}$.
	\item \textit{time(e)} is the timestamp associated to an event $e \in \mathcal{E}$.
\end{itemize}


\begin{mydefinition}{Business process perspectives}
	\\%Given a event log $\mathcal{L}$ with attributes $\mathcal{A}$; 
	A perspective $\Pi_{a_1, ..., a_n}(c)$ is the projection on one or multiple attributes $a_1, ..., a_n \in \mathcal{A^{*}}$ for one case $c \in \mathcal{C}$ in $\mathcal{L}$. Analogous, $\Pi_{a_1, ..., a_n}(L)$ is the perspective on $a_1, ..., a_n$ for all cases in $\mathcal{L}$. 
	%The control-flow perspective on the complete event log therefore is $C_{activity}$ (or simply $C$ if $A = \emptyset$). 
	%$p_{temporal}$ is alike defined as the extraction of attribute $a_{time}$. 
	%If more data for events are available there can also be a perspective on them called $p_{data}$, e.g., for costs.
\end{mydefinition}
Note that a perspective can also be a projection on a case attribute $a \in \mathscr{C}$. In the following, we frequently use the following perspectives:\\
The control-flow perspective $\Pi_{control-flow}$ as a projection on \textit{activity}, the resource perspective $\Pi_{resource}$ and the temporal perspective $\Pi_{time}$.


%\subsection{Encoding Techniques for Business Process Data}
%Depending on the data, task and technique, different encoding techniques are used when preparing event log data. The most common encoding techniques for machine-learning-based methods are presented below.

%\paragraph{Integer Encoding}
%Assign each attribute value a unique integer $int \in [0, 1, 2, .., |\mathcal{V}_{a}|-1]$.\\
%$INT: \mathcal{V}_{a} \rightarrow int$%x \in [0, 1, 2, .., |\mathcal{V}_{a}|-1]$
%E.g. ["File travel request", "decide on approval requirements", "book travel"] $\rightarrow$ [0, 1, 2]

%\paragraph{One-Hot Encoding}
%Encode each label as a one-hot vector. That is a vector $ohe \in \{0, 1\}^{|\mathcal{V}_{a}|}$ filled with zeros but the i-th entry set to 1 such that each $v \in \mathcal{V}$ results in a unique $ohe$.\\
%$OHE: \mathcal{V}_{a} \rightarrow ohe$%x^{|\mathcal{V}_{a}|}$
%E.g. ["File travel request", "decide on approval requirements", "book travel"] $\rightarrow$ [[1, 0, 0], [0, 1, 0], [0, 0, 1]].

%\paragraph{Embedding}
%Embed each label in a n-dimensional vector space $emb \in \mathbb{R}^{n}$.\\
%$EMB: \mathcal{V}_{a} \rightarrow emb$

%\paragraph{Image encoding}
%Encode one multiple perspectives $\Pi$ to a single or multiple matrices $M^{h \times w \times c}$ of size $height \times width \times \#channels$.\\
%$IMG: \Pi_{a1, .., an} \rightarrow \{m \mid m \in M^{h \times w \times c}\}$

%\paragraph{Relative time}
%Temporal attributes in form of timestamps are often transformed to relative times, e.g. seconds after a certain point in time. Let $z(v_{1}, v_{2})$ be a function that calculates the seconds between $v_{1}$ and $v_{2}$ and $rel \in [0, max(\mathcal{V_{time}})$.
%$REL: \mathcal{V}_{time} \rightarrow rel$

%\subsection{Predictive Process Analystics}
%Predictive business process analytics summarizes predictive tasks on business process data recorded as event logs like business process prediction, business process monitoring, business process anomaly detection. In the following, we will give a formal definition of some of these tasks.

